Semi-Supervised Contrastive Learning with Orthonormal Prototypes

Contrastive learning has emerged as a powerful method in deep learning, excelling at learning effective representations through contrasting samples from different distributions. However, dimensional collapse, where embeddings converge into a lower-dimensional space, poses a significant challenge, especially in semi-supervised and self-supervised setups. In this paper, we first identify a critical learning-rate threshold, beyond which standard contrastive losses converge to collapsed solutions. Building on these insights, we propose CLOP, a novel semi-supervised loss function designed to prevent dimensional collapse by promoting the formation of orthogonal linear subspaces among class embeddings. Through extensive experiments on real and synthetic datasets, we demonstrate that CLOP improves performance in image classification and object detection tasks while also exhibiting greater stability across different learning rates and batch sizes.

==> 3.2-DimCollapse.tex <==
% \clearpage
\subsection{Cosine-Similarity Causes Dimensional Collapse}
There are three widely discussed methods for arranging $k$ {class embeddings} in an $m$-dimensional space, where $m \geq k$, to achieve optimal spatial utility.
The first method is the Simplex Equiangular Tight Frame (ETF), as introduced in \cite{zhu2021geometric, graf2021dissecting}. This approach arranges the vectors on a hyperplane such that all vectors are equidistant from each other. ETF is frequently used to explain the phenomenon of dimensional collapse observed in the final layer of a neural network.
The second method involves arranging $k$ vectors to be mutually orthogonal. 
The third method divides the $k$ vectors into equal-sized groups, where within each group, the vectors form pairs that point in opposite directions. Additionally, the vectors from different groups are orthogonal to each other.


\label{sec:dim_collapse}


While the second \textit{"orthogonal"} method yields the most distinguishable classes from a linear algebra standpoint, the first \textit{"simplex ETF"} and third \textit{"inverted groups"} methods achieve the optimal value of the InfoNCE-equivalent $\mathcal{L}_{\text{class}}$, given as $-k$. This result is obtained under the same conditions outlined in Section \ref{sec:complete_collapse}, where the model effectively consolidates samples from the same class into a unified {class embedding}.
However, none of these configurations are commonly observed in contrastive learning via gradient descent. Instead, a more common outcome is that the initially full-rank embedding space gradually collapses into a lower-dimensional subspace, where the embeddings are no longer equidistant. In this section, we take a microscopic perspective to explore how individual embeddings adjust to minimize total cosine similarity.

% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     %\vspace{-0.5cm}
%     \includegraphics[width=\linewidth]{Figures/svd_d100.pdf}
%     \includegraphics[width=\linewidth]{Figures/count_d100.pdf}
%     %\vspace{-0.8cm}
% \caption{Numerical experiments conducted in a 100-dimensional space with $k$ class embeddings. The results demonstrate that minimizing total cosine similarity via gradient descent leads to convergence within a subspace of rank $k-1$ (\textbf{upper plot}), without maintaining equal distances between the vectors (\textbf{lower plot}).}
%     \label{fig:svd100}
%     %\vspace{-0.6cm}
% \end{wrapfigure}

\begin{figure*}
    \centering
    % %\vspace{-0.5cm}
    \includegraphics[height=0.217\linewidth]{Figures/svd_d100.pdf}
    \includegraphics[height=0.217\linewidth]{Figures/count_d100.pdf}
    % %\vspace{-0.75cm}
\caption{{Numerical experiments illustrating dimensional collapse with $k$ class embeddings. The results show that minimizing total cosine similarity via gradient descent leads to convergence within a subspace of rank $k-1$ (\textbf{left}), while failing to preserve equal distances between the vectors (\textbf{right}).}}
    \label{fig:svd100}
    % %\vspace{-0.6cm}
\end{figure*}
This observation is validated by a simple numerical experiment, where we minimize the pairwise cosine similarity $\mathcal{L}_{\text{class}}$ among all {class embeddings} using gradient descent. The {class embeddings} are randomly initialized from a Gaussian distribution and normalized to unit norm at each iteration. As shown in Figure~\ref{fig:svd100}, the results demonstrate that gradient descent consistently converges to a subspace of rank $k-1$, where the pairwise similarities vary significantly.

Building on this observation, we present Lemma~\ref{theory-subspace} to illustrate that, in the case of full rank, the optimal movement for each individual {class embedding} is to align itself within the subspace spanned by all other {class embeddings}. Consequently, the {class embedding} closest to the others is most likely to be pushed into this subspace, eventually reaching a local optimum by forming a zero-mean subspace of rank $k-1$.

\begin{framed}
\begin{lemma}
    Let $\X = \{\x_1, \x_2, \dots, \x_{k-1}\}$ be a set of $k-1$ linearly-independent unit-norm {class embeddings} in an $m$-dimensional space, where $m \geq k$. The optimal arrangement of the additional individual {class embedding} $\x_k$ that minimize the total cosine similarity score $\L_{class}$ (\eqref{eq-total-cossim}) will result in $\x_k$ being linearly dependent on the remaining {class embeddings} in $\X$.
    \label{theory-subspace}
\end{lemma}
\end{framed}

Lemma~\ref{theory-subspace} can be proven by constructing two matrices, $\mathbf{X}$ and $\mathbf{X}'$, each consisting of $k$ vectors. One matrix is full rank, while the other has rank $k-1$. The only difference between $\mathbf{X}$ and $\mathbf{X}'$ is that the vector $\mathbf{x}_k$ in $\mathbf{X}$ lies in a distinct dimension, whereas $\mathbf{x}'_k$ in $\mathbf{X}'$ is the normalized projection of $\mathbf{x}_k$ onto the subspace spanned by the remaining vectors in both $\mathbf{X}$ and $\mathbf{X}'$. It can be shown that $\mathcal{L}_{\text{class}}(\mathbf{X}) > \mathcal{L}_{\text{class}}(\mathbf{X}')$. The complete proof is provided in Appendix~\ref{proof3}.

==> raw-table-11_27_2024.tex <==

\section{Tiny-ImageNet}
\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.629 & 0.661 & 0.683 & 0.701 & 0.708 & 0.696 & 0.659 \\
SupCon & 0.458 & 0.472 & 0.482 & 0.485 & 0.488 & 0.488 & 0.504 \\
SupCon-10\% & 0.454 & 0.462 & 0.476 & 0.475 & 0.475 & 0.473 & 0.481 \\
SupCon-50\% & 0.452 & 0.465 & 0.477 & 0.487 & 0.482 & 0.475 & 0.485 \\
SupCon-OAR-10\% & 0.554 & 0.592 & 0.615 & 0.636 & 0.646 & 0.643 & 0.648 \\
SupCon-OAR-50\% & 0.620 & 0.662 & 0.679 & 0.695 & 0.708 & 0.691 & 0.679 \\
ETF & 0.615 & 0.633 & 0.664 & 0.675 & 0.692 & 0.672 & 0.642 \\
ETF-10\% & 0.527 & 0.575 & 0.603 & 0.620 & 0.624 & 0.626 & 0.633 \\
ETF-50\% & 0.603 & 0.644 & 0.659 & 0.669 & 0.689 & 0.667 & 0.657 \\
VICReg & 0.486 & 0.501 & 0.519 & 0.521 & 0.525 & 0.525 & 0.536 \\
VICReg-Supcon & 0.494 & 0.504 & 0.526 & 0.534 & 0.533 & 0.538 & 0.546 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.865 & 0.845 & 0.888 & 0.897 & 0.906 & 0.900 & 0.878 \\
SupCon & 0.721 & 0.738 & 0.747 & 0.756 & 0.759 & 0.756 & 0.766 \\
SupCon-10\% & 0.722 & 0.729 & 0.742 & 0.740 & 0.740 & 0.740 & 0.748 \\
SupCon-50\% & 0.715 & 0.733 & 0.746 & 0.747 & 0.747 & 0.743 & 0.747 \\
SupCon-OAR-10\% & 0.823 & 0.847 & 0.866 & 0.883 & 0.883 & 0.883 & 0.889 \\
SupCon-OAR-50\% & 0.864 & 0.887 & 0.890 & 0.910 & 0.910 & 0.900 & 0.891 \\
ETF & 0.845 & 0.831 & 0.859 & 0.878 & 0.880 & 0.889 & 0.849 \\
ETF-10\% & 0.800 & 0.826 & 0.839 & 0.872 & 0.865 & 0.869 & 0.878 \\
ETF-50\% & 0.834 & 0.867 & 0.863 & 0.887 & 0.899 & 0.876 & 0.879 \\
VICReg & 0.729 & 0.743 & 0.777 & 0.769 & 0.773 & 0.782 & 0.785 \\
VICReg-Supcon & 0.745 & 0.752 & 0.774 & 0.776 & 0.785 & 0.792 & 0.795 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.451 & 0.703 & 0.696 & 0.664 & 0.635 & 0.622 & 0.606 & 0.578 \\
SupCon & 0.419 & 0.487 & 0.488 & 0.483 & 0.477 & 0.470 & 0.475 & 0.282 \\
SupCon-10\% & 0.413 & 0.476 & 0.473 & 0.469 & 0.465 & 0.463 & 0.455 & 0.276 \\
SupCon-50\% & 0.411 & 0.479 & 0.475 & 0.475 & 0.467 & 0.468 & 0.468 & 0.275 \\
SupCon-OAR-10\% & 0.424 & 0.638 & 0.643 & 0.647 & 0.644 & 0.631 & 0.624 & 0.507 \\
SupCon-OAR-50\% & 0.442 & 0.704 & 0.691 & 0.673 & 0.633 & 0.604 & 0.598 & 0.577 \\
ETF & 0.435 & 0.686 & 0.681 & 0.650 & 0.624 & 0.598 & 0.589 & 0.549 \\
ETF-10\% & 0.399 & 0.624 & 0.630 & 0.628 & 0.619 & 0.606 & 0.598 & 0.486 \\
ETF-50\% & 0.431 & 0.685 & 0.680 & 0.656 & 0.613 & 0.589 & 0.585 & 0.567 \\
VICReg & 0.419 & 0.551 & 0.548 & 0.516 & 0.516 & 0.478 & 0.449 & 0.223 \\
VICReg-Supcon & 0.450 & 0.614 & 0.591 & 0.563 & 0.544 & 0.538 & 0.511 & 0.244 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.719 & 0.909 & 0.900 & 0.878 & 0.856 & 0.835 & 0.782 & 0.853 \\
SupCon & 0.686 & 0.751 & 0.756 & 0.749 & 0.743 & 0.740 & 0.740 & 0.547 \\
SupCon-10\% & 0.678 & 0.745 & 0.740 & 0.737 & 0.735 & 0.729 & 0.720 & 0.541 \\
SupCon-50\% & 0.672 & 0.747 & 0.743 & 0.742 & 0.734 & 0.731 & 0.720 & 0.538 \\
SupCon-OAR-10\% & 0.694 & 0.884 & 0.883 & 0.890 & 0.883 & 0.876 & 0.871 & 0.776 \\
SupCon-OAR-50\% & 0.707 & 0.912 & 0.900 & 0.869 & 0.854 & 0.838 & 0.834 & 0.837 \\
ETF & 0.698 & 0.881 & 0.887 & 0.862 & 0.832 & 0.816 & 0.769 & 0.831 \\
ETF-10\% & 0.673 & 0.871 & 0.860 & 0.874 & 0.867 & 0.856 & 0.856 & 0.749 \\
ETF-50\% & 0.679 & 0.886 & 0.875 & 0.859 & 0.828 & 0.822 & 0.819 & 0.807 \\
VICReg & 0.684 & 0.792 & 0.817 & 0.784 & 0.763 & 0.730 & 0.700 & 0.459 \\
VICReg-Supcon & 0.784 & 0.853 & 0.850 & 0.824 & 0.802 & 0.783 & 0.751 & 0.500 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\section{Cifar100}
\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.723 & 0.723 & 0.696 & 0.720 & 0.733 & 0.754 & 0.746 \\
SupCon & 0.567 & 0.601 & 0.666 & 0.716 & 0.715 & 0.733 & 0.734 \\
SupCon-10\% & 0.524 & 0.517 & 0.554 & 0.581 & 0.591 & 0.595 & 0.606 \\
SupCon-50\% & 0.539 & 0.587 & 0.615 & 0.618 & 0.628 & 0.625 & 0.655 \\
SupCon-OAR-10\% & 0.601 & 0.648 & 0.664 & 0.683 & 0.703 & 0.665 & 0.634 \\
SupCon-OAR-50\% & 0.699 & 0.707 & 0.742 & 0.760 & 0.744 & 0.737 & 0.725 \\
ETF & 0.695 & 0.696 & 0.668 & 0.701 & 0.715 & 0.731 & 0.723 \\
ETF-10\% & 0.574 & 0.633 & 0.646 & 0.663 & 0.677 & 0.654 & 0.623 \\
ETF-50\% & 0.681 & 0.691 & 0.731 & 0.730 & 0.734 & 0.712 & 0.711 \\
VICReg & 0.546 & 0.556 & 0.589 & 0.599 & 0.627 & 0.613 & 0.630 \\
VICReg-Supcon & 0.575 & 0.611 & 0.647 & 0.650 & 0.663 & 0.648 & 0.694 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.927 & 0.923 & 0.920 & 0.924 & 0.927 & 0.938 & 0.937 \\
SupCon & 0.846 & 0.872 & 0.903 & 0.921 & 0.922 & 0.935 & 0.936 \\
SupCon-10\% & 0.813 & 0.814 & 0.841 & 0.857 & 0.865 & 0.865 & 0.874 \\
SupCon-50\% & 0.819 & 0.835 & 0.856 & 0.866 & 0.884 & 0.884 & 0.894 \\
SupCon-OAR-10\% & 0.868 & 0.892 & 0.874 & 0.894 & 0.903 & 0.904 & 0.891 \\
SupCon-OAR-50\% & 0.899 & 0.907 & 0.889 & 0.920 & 0.906 & 0.910 & 0.906 \\
ETF & 0.905 & 0.907 & 0.892 & 0.906 & 0.908 & 0.917 & 0.918 \\
ETF-10\% & 0.844 & 0.878 & 0.849 & 0.874 & 0.887 & 0.892 & 0.869 \\
ETF-50\% & 0.881 & 0.880 & 0.861 & 0.901 & 0.882 & 0.885 & 0.894 \\
VICReg & 0.833 & 0.825 & 0.858 & 0.851 & 0.871 & 0.871 & 0.886 \\
VICReg-Supcon & 0.874 & 0.889 & 0.875 & 0.894 & 0.898 & 0.892 & 0.900 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.565 & 0.744 & 0.744 & 0.749 & 0.747 & 0.754 & 0.750 & 0.657 \\
SupCon & 0.548 & 0.739 & 0.745 & 0.746 & 0.736 & 0.733 & 0.720 & 0.543 \\
SupCon-10\% & 0.458 & 0.583 & 0.601 & 0.611 & 0.601 & 0.595 & 0.582 & 0.477 \\
SupCon-50\% & 0.503 & 0.611 & 0.647 & 0.660 & 0.652 & 0.647 & 0.625 & 0.527 \\
SupCon-OAR-10\% & 0.478 & 0.649 & 0.664 & 0.656 & 0.669 & 0.665 & 0.638 & 0.606 \\
SupCon-OAR-50\% & 0.540 & 0.726 & 0.748 & 0.741 & 0.746 & 0.728 & 0.714 & 0.682 \\
ETF & 0.547 & 0.734 & 0.728 & 0.738 & 0.728 & 0.725 & 0.736 & 0.644 \\
ETF-10\% & 0.458 & 0.628 & 0.652 & 0.627 & 0.657 & 0.636 & 0.621 & 0.578 \\
ETF-50\% & 0.515 & 0.709 & 0.732 & 0.714 & 0.734 & 0.716 & 0.692 & 0.667 \\
VICReg & 0.515 & 0.645 & 0.643 & 0.615 & 0.609 & 0.572 & 0.540 & 0.325 \\
VICReg-Supcon & 0.547 & 0.709 & 0.693 & 0.672 & 0.651 & 0.642 & 0.601 & 0.344 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.835 & 0.929 & 0.929 & 0.935 & 0.932 & 0.938 & 0.935 & 0.875 \\
SupCon & 0.832 & 0.928 & 0.931 & 0.937 & 0.931 & 0.934 & 0.928 & 0.825 \\
SupCon-10\% & 0.756 & 0.860 & 0.874 & 0.876 & 0.870 & 0.865 & 0.859 & 0.774 \\
SupCon-50\% & 0.790 & 0.894 & 0.906 & 0.905 & 0.885 & 0.884 & 0.884 & 0.808 \\
SupCon-OAR-10\% & 0.771 & 0.894 & 0.902 & 0.906 & 0.906 & 0.904 & 0.889 & 0.870 \\
SupCon-OAR-50\% & 0.770 & 0.899 & 0.916 & 0.913 & 0.905 & 0.910 & 0.902 & 0.895 \\
ETF & 0.817 & 0.912 & 0.914 & 0.919 & 0.921 & 0.917 & 0.908 & 0.851 \\
ETF-10\% & 0.758 & 0.870 & 0.883 & 0.883 & 0.884 & 0.882 & 0.872 & 0.844 \\
ETF-50\% & 0.751 & 0.873 & 0.887 & 0.902 & 0.888 & 0.890 & 0.886 & 0.874 \\
VICReg & 0.721 & 0.858 & 0.846 & 0.816 & 0.812 & 0.780 & 0.749 & 0.533 \\
VICReg-Supcon & 0.750 & 0.920 & 0.883 & 0.870 & 0.838 & 0.829 & 0.817 & 0.548 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\section{ImageNet}
\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.790 & 0.805 & 0.810 & 0.802 & 0.815 & 0.836 & 0.850 \\
SupCon & 0.560 & 0.610 & 0.659 & 0.688 & 0.731 & 0.747 & 0.769 \\
SupCon-10\% & 0.512 & 0.525 & 0.587 & 0.625 & 0.651 & 0.672 & 0.704 \\
SupCon-50\% & 0.545 & 0.575 & 0.604 & 0.653 & 0.676 & 0.710 & 0.734 \\
SupCon-OAR-10\% & 0.701 & 0.706 & 0.724 & 0.730 & 0.756 & 0.768 & 0.791 \\
SupCon-OAR-50\% & 0.769 & 0.784 & 0.792 & 0.788 & 0.794 & 0.811 & 0.829 \\
ETF & 0.779 & 0.791 & 0.792 & 0.782 & 0.805 & 0.815 & 0.828 \\
ETF-10\% & 0.677 & 0.692 & 0.697 & 0.701 & 0.744 & 0.753 & 0.774 \\
ETF-50\% & 0.748 & 0.763 & 0.771 & 0.766 & 0.764 & 0.798 & 0.806 \\
VICReg & 0.525 & 0.524 & 0.598 & 0.621 & 0.637 & 0.668 & 0.713 \\
VICReg-Supcon & 0.556 & 0.597 & 0.622 & 0.662 & 0.696 & 0.737 & 0.743 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Batch Sizes and Methods}
\begin{tabular}{lccccccc}
\hline
\textbf{Category} & \multicolumn{7}{c}{\textbf{Batch Size}} \\
\cline{2-8}
 & 32 & 64 & 128 & 256 & 512 & 1024 & 2048 \\
\hline
SupCon-OAR & 0.924 & 0.944 & 0.947 & 0.918 & 0.948 & 0.959 & 0.983 \\
SupCon & 0.702 & 0.738 & 0.776 & 0.812 & 0.875 & 0.886 & 0.907 \\
SupCon-10\% & 0.688 & 0.702 & 0.734 & 0.777 & 0.809 & 0.851 & 0.874 \\
SupCon-50\% & 0.638 & 0.646 & 0.723 & 0.746 & 0.781 & 0.789 & 0.830 \\
SupCon-OAR-10\% & 0.837 & 0.848 & 0.857 & 0.852 & 0.892 & 0.900 & 0.927 \\
SupCon-OAR-50\% & 0.896 & 0.928 & 0.927 & 0.923 & 0.923 & 0.937 & 0.949 \\
ETF & 0.910 & 0.918 & 0.927 & 0.905 & 0.930 & 0.930 & 0.962 \\
ETF-10\% & 0.808 & 0.824 & 0.837 & 0.829 & 0.873 & 0.882 & 0.913 \\
ETF-50\% & 0.867 & 0.909 & 0.909 & 0.913 & 0.894 & 0.918 & 0.927 \\
VICReg & 0.661 & 0.678 & 0.738 & 0.752 & 0.802 & 0.809 & 0.863 \\
VICReg-Supcon & 0.719 & 0.734 & 0.782 & 0.829 & 0.851 & 0.884 & 0.874 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-1 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.418 & 0.817 & 0.826 & 0.832 & 0.841 & 0.836 & 0.831 & 0.679 \\
SupCon & 0.412 & 0.678 & 0.707 & 0.729 & 0.739 & 0.747 & 0.730 & 0.526 \\
SupCon-10\% & 0.435 & 0.630 & 0.642 & 0.664 & 0.673 & 0.672 & 0.659 & 0.232 \\
SupCon-50\% & 0.478 & 0.644 & 0.660 & 0.682 & 0.701 & 0.710 & 0.693 & 0.318 \\
SupCon-OAR-10\% & 0.443 & 0.739 & 0.743 & 0.741 & 0.750 & 0.768 & 0.751 & 0.512 \\
SupCon-OAR-50\% & 0.472 & 0.803 & 0.813 & 0.801 & 0.810 & 0.811 & 0.795 & 0.584 \\
ETF & 0.403 & 0.797 & 0.805 & 0.806 & 0.819 & 0.819 & 0.809 & 0.658 \\
ETF-10\% & 0.432 & 0.720 & 0.718 & 0.725 & 0.737 & 0.756 & 0.739 & 0.499 \\
ETF-50\% & 0.451 & 0.776 & 0.797 & 0.779 & 0.796 & 0.801 & 0.780 & 0.558 \\
VICReg & 0.528 & 0.676 & 0.681 & 0.621 & 0.634 & 0.615 & 0.579 & 0.361 \\
VICReg-Supcon & 0.579 & 0.747 & 0.721 & 0.695 & 0.696 & 0.662 & 0.611 & 0.380 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

\begin{table}[htbp]
\centering
\caption{Top-5 Accuracy Results Across Different Learning Rates and Methods}
\begin{tabular}{lccccccccc}
\hline
\textbf{Category} & \multicolumn{8}{c}{\textbf{Learning Rate}} \\
\cline{2-9}
 & 0.1 & 0.8 & 1.2 & 1.6 & 2.0 & 2.4 & 2.8 & 10.0 \\
\hline
SupCon-OAR & 0.562 & 0.971 & 0.966 & 0.958 & 0.987 & 0.993 & 0.961 & 0.808 \\
SupCon & 0.563 & 0.835 & 0.851 & 0.878 & 0.896 & 0.875 & 0.885 & 0.650 \\
SupCon-10\% & 0.575 & 0.770 & 0.787 & 0.818 & 0.796 & 0.830 & 0.784 & 0.415 \\
SupCon-50\% & 0.601 & 0.769 & 0.795 & 0.802 & 0.841 & 0.864 & 0.813 & 0.469 \\
SupCon-OAR-10\% & 0.585 & 0.870 & 0.893 & 0.874 & 0.879 & 0.925 & 0.880 & 0.649 \\
SupCon-OAR-50\% & 0.606 & 0.936 & 0.960 & 0.943 & 0.929 & 0.946 & 0.940 & 0.707 \\
ETF & 0.541 & 0.955 & 0.949 & 0.947 & 0.973 & 0.975 & 0.949 & 0.798 \\
ETF-10\% & 0.555 & 0.847 & 0.875 & 0.844 & 0.851 & 0.911 & 0.859 & 0.638 \\
ETF-50\% & 0.586 & 0.922 & 0.936 & 0.928 & 0.915 & 0.933 & 0.911 & 0.690 \\
VICReg & 0.724 & 0.855 & 0.864 & 0.807 & 0.808 & 0.777 & 0.743 & 0.529 \\
VICReg-Supcon & 0.756 & 0.925 & 0.911 & 0.894 & 0.856 & 0.831 & 0.805 & 0.569 \\
\hline
\end{tabular}
\label{tab:accuracy_results}
\end{table}

==> raw-tables.tex <==
\clearpage
\subsection{Semi-Supervised Learning with $50\%$ Labels}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Cifar100 &0.601 &0.648 &0.664 &0.683 &0.703 &0.665 &0.634\\ \hline
InfoNCE on Cifar100 &0.524 &0.517 &0.554 &0.581 &0.591 &0.595 &0.606\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.620 &0.662 &0.679 &0.695 &0.708 &0.691 &0.679\\ \hline
InfoNCE on Tiny-ImageNet &0.452 &0.465 &0.477 &0.487 &0.482 &0.475 &0.485\\ \hline
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Cifar100 &0.868 &0.892 &0.874 &0.894 &0.903 &0.904 &0.891\\ \hline
InfoNCE on Cifar100 &0.813 &0.814 &0.841 &0.857 &0.865 &0.865 &0.874\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.864 &0.887 &0.890 &0.91 &0.91 &0.9 &0.891\\ \hline
InfoNCE on Tiny-ImageNet &0.715 &0.733 &0.746 &0.747 &0.747 &0.743 &0.747\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning Rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Cifar100 &0.478 &0.649 &0.664 &0.656 &0.669 &0.665 &0.638 &0.606\\ \hline
InfoNCE on Cifar100 &0.458 &0.583 &0.601 &0.611 &0.601 &0.595 &0.582 &0.477\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.442 &0.704 &0.691 &0.673 &0.633 &0.604 &0.598 &0.577\\ \hline
InfoNCE on Tiny-ImageNet &0.411 &0.479 &0.475 &0.475 &0.467 &0.468 &0.468 &0.275\\ \hline
\end{tabular}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Cifar100 &0.771 &0.894 &0.902 &0.906 &0.906 &0.904 &0.889 &0.87\\ \hline
InfoNCE on Cifar100 &0.756 &0.86 &0.874 &0.876 &0.87 &0.865 &0.859 &0.774\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.707 &0.912 &0.9 &0.869 &0.854 &0.838 &0.834 &0.837\\ \hline
InfoNCE on Tiny-ImageNet &0.672 &0.747 &0.743 &0.742 &0.734 &0.731 &0.720 &0.538\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\clearpage
\subsection{Semi-Supervised Learning with $10\%$ Labels (only on Tiny-Imagenet)}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.554 &0.592 &0.615 &0.636 &0.646 &0.643 &0.648\\ \hline
InfoNCE on Tiny-ImageNet &0.454 &0.462 &0.476 &0.475 &0.475 &0.473 &0.481\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs batch size.}
% \end{table}


% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.823 &0.847 &0.866 &0.883 &0.883 &0.883 &0.889\\ \hline
InfoNCE on Tiny-ImageNet &0.722 &0.729 &0.742 &0.74 &0.74 &0.74 &0.748\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning Rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.424 &0.638 &0.643 &0.647 &0.644 &0.631 &0.624 &0.507\\ \hline
InfoNCE on Tiny-ImageNet &0.413 &0.476 &0.473 &0.469 &0.465 &0.463 &0.455 &0.276\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs lr.}
% \end{table}

% \begin{table}
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.694 &0.884 &0.883 &0.89 &0.883 &0.876 &0.871 &0.776\\ \hline
InfoNCE on Tiny-ImageNet &0.678 &0.745 &0.740 &0.737 &0.735 &0.729 &0.72 &0.541\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\clearpage
\subsection{Fully-Supervised Learning}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
SupCon-OAR on Cifar100 &0.723 &0.723 &0.696 &0.720 &0.733 &0.754 &0.746\\ \hline
SupCon on Cifar100 &0.567 &0.601 &0.666 &0.716 &0.715 &0.733 &0.734\\ \hline
SupCon-OAR on Tiny-ImageNet &0.629 &0.661 &0.683 &0.701 &0.708 &0.696 &0.659\\ \hline
SupCon on Tiny-ImageNet &0.458 &0.472 &0.482 &0.485 &0.488 &0.488 &0.504\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs batch size.}
% \end{table}

% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
SupCon-OAR on Cifar100 &0.927 &0.923 &0.92 &0.924 &0.927 &0.938 &0.936\\ \hline
SupCon on Cifar100 &0.846 &0.872 &0.903 &0.921 &0.922 &0.935 &0.936\\ \hline
SupCon-OAR on Tiny-ImageNet &0.865 &0.845 &0.888 &0.897 &0.906 &0.9 &0.878\\ \hline
SupCon on Tiny-ImageNet &0.721 &0.738 &0.747 &0.756 &0.759 &0.756 &0.766\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
SupCon-OAR on Cifar100 &0.565 &0.744 &0.744 &0.749 &0.747 &0.754 &0.75 &0.657\\ \hline
SupCon on Cifar100 &0.548 &0.739 &0.745 &0.746 &0.736 &0.733 &0.720 &0.543\\ \hline
SupCon-OAR on Tiny-ImageNet &0.451 &0.703 &0.696 &0.664 &0.635 &0.622 &0.606 &0.578\\ \hline
SupCon on Tiny-ImageNet &0.419 &0.487 &0.488 &0.483 &0.477 &0.47 &0.475 &0.282\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs lr.}
% \end{table}

% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
SupCon-OAR on Cifar100 &0.835 &0.929 &0.929 &0.935 &0.932 &0.938 &0.935 &0.875\\ \hline
SupCon on Cifar100 &0.832 &0.928 &0.931 &0.937 &0.931 &0.934 &0.928 &0.825\\ \hline
SupCon-OAR on Tiny-ImageNet &0.719 &0.809 &0.9 &0.878 &0.856 &0.835 &0.782 &0.853\\ \hline
SupCon on Tiny-ImageNet &0.686 &0.751 &0.756 &0.749 &0.743 &0.74 &0.74 &0.547\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Similarity Metric} &\textbf{Top-1 Cifar100} &\textbf{Top-5 Cifar100} &\textbf{Top-1 Tiny-Imagenet} &\textbf{Top-5 Tiny-Imagenet}\\ \hline
Cosine &0.754 &0.938 &0.595 &0.845\\ \hline
Euclidean &0.749 &0.933 &0.588 &0.839\\ \hline
Manhattan &0.715 &0.899 &0.659 &0.878\\ \hline
\end{tabular}
\caption{Accuracy of different distance method, train on SupCon-OAR. Cifar100 is trained on 1024, and Tiny-Imagenet is trained on 2048}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Augmentation} &\textbf{Top-1 Accuracy} &\textbf{Top-5 Accuracy}\\ \hline
RandAug &0.696 &0.9 \\ \hline
AutoAug-Imagenet &0.546 &0.776\\ \hline
SimCLR-like Augmentation &0.499 &0.77\\ \hline
\end{tabular}
\caption{Accuracy of different augmentation method on Tiny ImageNet. It is shown that the Random Augmentation yield the best result for both Top-1 and Top-5. The results are trained on batch size 1024.}
\end{table}



\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Similarity Metric} &\textbf{Top-1 Cifar100} &\textbf{Top-5 Cifar100} &\textbf{Top-1 Tiny-Imagenet} &\textbf{Top-5 Tiny-Imagenet}\\ \hline
Cosine &0.754 &0.938 &0.595 &0.845\\ \hline
Euclidean &0.749 &0.933 &0.588 &0.839\\ \hline
Manhattan &0.715 &0.899 &0.659 &0.878\\ \hline
\end{tabular}
\caption{Accuracy of different distance method, train on SupCon-OAR. Cifar100 is trained on 1024, and Tiny-Imagenet is trained on 2048}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Augmentation} &\textbf{Top-1 Accuracy} &\textbf{Top-5 Accuracy}\\ \hline
RandAug &0.696 &0.9 \\ \hline
AutoAug-Imagenet &0.546 &0.776\\ \hline
SimCLR-like Augmentation &0.499 &0.77\\ \hline
\end{tabular}
\caption{Accuracy of different augmentation method on Tiny ImageNet. It is shown that the Random Augmentation yield the best result for both Top-1 and Top-5. The results are trained on batch size 1024.}
\end{table}

